HAVE-FUN: Human Avatar Reconstruction from Few-Shot Unconstrained Images

As for human avatar reconstruction, contemporary techniques commonly necessitate the acquisition of costly data and struggle to achieve satisfactory results from a small number of casual images. In this paper, we investigate this task from a few-shot unconstrained photo album. The reconstruction of human avatars from such data sources is challenging because of limited data amount and dynamic articulated poses. For handling dynamic data, we integrate a skinning mechanism with deep marching tetrahedra (DMTet) to form a drivable tetrahedral representation, which drives arbitrary mesh topologies generated by the DMTet for the adaptation of unconstrained images. To effectively mine instructive information from few-shot data, we devise a two-phase optimization method with few-shot reference and few-shot guidance. The former focuses on aligning avatar identity with reference images, while the latter aims to generate plausible appearances for unseen regions. Overall, our framework, called HaveFun, can undertake avatar reconstruction, rendering, and animation. Extensive experiments on our developed benchmarks demonstrate that HaveFun exhibits substantially superior performance in reconstructing the human body and hand. Project website: https://seanchenxy.github.io/HaveFunWeb/.

==> Figures/fig_bodyseq.tex <==
\begin{figure*}[h]
\begin{center}
\includegraphics[width=0.9\linewidth]{Images/bodyseq.pdf}
\caption{Animation sequences of human bodies. Please refer to \textit{suppl. video} for dynamic results.
}
\label{fig:bodyseq}
\end{center}
\vspace{-0.3cm}
\end{figure*}

==> Figures/fig_handseq.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{Images/handseq.pdf}
\caption{Animation sequences of hands. Please refer to \textit{suppl. video} for dynamic results.
}
\label{fig:handseq}
\end{center}
\vspace{-0.3cm}
\end{figure*}

==> Figures/fig_lapvn.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.95\linewidth]{Images/lapvn.png}
\caption{Ablation study on the Laplacian normal constraint. 
}
\label{fig:lapvn}
\end{center}
\vspace{-0.3cm}
\end{figure}

==> Figures/fig_realbody.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{Images/realbody.pdf}
\caption{Results on few-shot unconstrained captures. Training images are captured by us. Please refer to \textit{suppl. video} for dynamic results.
}
\label{fig:realbody}
\end{center}
\vspace{-0.3cm}
\end{figure*}

==> Figures/fig_snapseq.tex <==
\begin{figure*}[h]
\begin{center}
\includegraphics[width=\linewidth]{Images/snapseq.pdf}
\caption{Results on few-shot unconstrained captures. Training images are from PeopleSnapShot \cite{bib:PeopleSnapShot}. Please refer to \textit{suppl. video} for dynamic results.
}
\label{fig:snapseq}
\end{center}
\vspace{-0.3cm}
\end{figure*}

==> Sections/0_abstract_old.tex <==
\begin{abstract}
For human avatar reconstruction, contemporary techniques commonly necessitate the acquisition of costly data and struggle to achieve satisfactory results from easily available data sources. 
In this paper, we investigate this task from few-shot photo album. 
The reconstruction of human avatars from such data sources is challenging because of the limited data amount (as few as 2 images), dynamic articulated poses, and varying expressions. 
To this end, we introduce a drivable tetrahedra representation to model human geometry. This allows the skinning mechanism to drive arbitrary mesh topologies generated by deep-marching tetrahedra.
Besides, a texture field is employed to produce realistic avatar texture. 
To optimize the above framework with few-shot data, we devise a two-phase optimization method with few-shot reference and few-shot guidance.
The former focuses on aligning avatar identity with reference images, while the latter aims to regularize the avatar rendering from various random viewpoints.
With the above strategies, the framework is evaluated on our developed benchmarks for the human body and hand. The results exhibit a substantial improvement over existing techniques.
Our models and datasets will be made publicly available.

\end{abstract}

==> Sections/1_intro_old.tex <==
\section{Introduction}
\label{sec:intro}
Human avatar reconstruction and rendering have experienced rapid development in recent years and shown great potential for AR/VR, metaverse, etc \cite{bib:handAR,bib:mobrecon}. %Tremendous research efforts have been made towards this task, including \cite{bib:IMAvatar,bib:SelfRecon,bib:HandAvatar,bib:TotalSelfScan}, to name a few.
One of the challenges in this field is the data collection. Previous works typically require an immense number of tailored data, including multi-view RGB video \cite{bib:NeuralBody}, monocular RGB video \cite{bib:HumanNeRF}, textured scan video \cite{bib:XAvatar}, image set \cite{bib:PersonNeRF}, etc. Acquiring those data is \textit{cumbersome, labor-intensive, or time-consuming}, and even depends on expensive devices. While an alternative research line can reconstruct humans using several images \cite{bib:PIFu}, the \textit{multi-view static} data required by this approach are also hard to capture.

%In certain situations, data acquisition is even infeasible, such as capturing oneself in one's youth. Hence, a question arises —— \textit{Is there any way to reconstruct animatable 3D avatars from a personalized album, even without a tailored data collection? This data source is featured by limited data quantity and unconstrained human behaviors}. The answer, as this paper will show, is arguably yes, if at least 2-viewpoint images can be founded. 

In some scenarios, acquiring data is even impossible, such as attempting to capture images of oneself from one's younger years, or of historic individuals such as Albert Einstein. This leads to a pivotal question: ``Is it feasible to reconstruct animatable 3D avatars from a personal photo album, even in the absence of a specifically curated data collection? The data in question here is characterized by its limited quantity and the unstructured nature of human behaviors it captures." As this paper will demonstrate, the answer leans toward the affirmative, especially if images from at least two different perspectives can be obtained.

From a technical perspective, the neural radiance field (NeRF) \cite{bib:NeRF} is normally employed as the predominant 3D representation for humans. We argue, however, that NeRF is intrinsically unsuitable for the few-shot setting. First, due to its static nature, NeRF is inherently ill-suited for handling articulated deformations. Although various motion fields \cite{bib:HumanNeRF,bib:SNARF,bib:SANeRF} are used to tackle this issue, accurately driving a volume space using limited data is an even harder problem.
Second, the few-shot task can benefit from priors, yet the quality of NeRF training with full-image prior, such as GAN \cite{bib:Mimic3D} or score distillation sampling (SDS) \cite{bib:DreamFusion}, is bounded by the memory bottleneck as it is inherently memory-hungry. Recently, deep marching tetrahedra (DMTet) \cite{bib:DMTet} proposes a hybrid method for static-scene representation, where the signed distance field (SDF) can be converted to drivable mesh through a differentiable process.
As it is memory-friendly and compatible with mesh driving, we are motivated to investigate a few-shot dynamic human reconstruction with the DMTet framework.

%Another primary focus of this field is to design 3D representations for the human, where neural radiance field (NeRF) \cite{bib:NeRF} is prevalently employed. However, NeRF is deemed unsuitable for the few-shot task. First, as the NeRF is a static representation, it is inherently ill-suited for handling articulated deformations. Although various motion fields \cite{bib:HumanNeRF,bib:SNARF,bib:SANeRF} are used to tackle this issue, accurately driving a volume space using limited data is an even harder problem.
%Second, the few-shot task can benefit from priors, yet the quality of NeRF training with full-image prior, such as GAN \cite{bib:Mimic3D} or score distillation sampling (SDS) \cite{bib:DreamFusion}, is bounded by the memory bottleneck as it is inherently memory-hungry. Recently, deep marching tetrahedra (DMTet) \cite{bib:DMTet} proposes a hybrid method for static-scene representation, where the signed distance field (SDF) can be converted to drivable mesh through a differentiable process.
%As it is memory-friendly and compatible with mesh driving, we are motivated to investigate a few-shot dynamic human reconstruction with the DMTet framework.

In this paper, we propose HaveFun, \textbf{H}uman \textbf{AV}atar r\textbf{E}construction from \textbf{F}ew-shot \textbf{UN}constrained images.
To this end, we build a 3D representation based on the tetrahedra grid and investigate multiple prior knowledge for human shape, motion, and unseen textures. 
First, we use skinning weights and blending shapes defined by SMPLX \cite{bib:SMPLX} to develop a drivable tetrahedra representation. Benefiting from this, we extend the traditional static-scene DMTet \cite{bib:Get3D,bib:DMTet} to model the articulated human body under a dynamic condition. Furthermore, it is conceived that the initialization is crucial for the few-shot task, and the driveable representation allows the use of canonical SMPLX shape as the prior to make the tetrahedra grid well-initialized. Additionally, to generate plausible textures for the unseen region, we use the SDS \cite{bib:DreamFusion,bib:SJC} technique to regularize the optimization process. Different from existing diffusion-based image-to-3D tasks that rely on textual descriptions or captions \cite{bib:RealFusion,bib:MakeIt3D}, we directly utilize the image as the prompt \cite{bib:Zero123} so that faithful visual feature can be preserved.

Note that the human body and hand have distinct properties. The body is characterized by intricate geometry (\eg, hair/cloth) and remarkable facial features, while the hand exhibits smooth bare geometry and subtle palm wrinkles. Unlike prior approaches that focus solely on either the body or the hand, our method is designed for both of them with a unified framework and subtle tailored designs. To this end, we develop benchmarks for both the human body and hand with the assistance of XHumans \cite{bib:XAvatar} and DART \cite{bib:DART}. %Also, freely collected images are employed for demonstration. 
As a result, our method can reconstruct human avatars with few-shot (as few as 2) images and achieve realistic rendering quality. Besides, we can perform avatar animation in various unseen human poses. 

Our main contributions are summarized as follows:
\begin{itemize}[leftmargin=*,topsep=3pt]
    \setlength\itemsep{0em}
    \item We achieve the human avatar reconstruction from \textit{few-shot unconstrained} images, a challenging task that has not been addressed in prior research. %As a result, we significantly enhance the practical significance of this research area.
    \item We explore a drivable tetrahedra representation for articulated motion and a diffusion model for non-static human reconstruction. Consequently, the DMTet and diffusion techniques are extended for dynamic 3D scenes.
    \item We develop benchmarks for few-shot dynamic body/hand reconstruction task. Extensive evaluations indicate our method outperforms prior arts by a large margin. 
\end{itemize}
% The principal contribution of this paper is to achieve the few-shot dynamic human reconstruction task. Additional technique contributions encompass the development of a drivable tetrahedra representation for articulated motion and the exploration of a diffusion model for non-static human reconstruction. A by-product of this paper is few-shot dynamic datasets for the human body and hand. 
We believe our endeavors would %streamline the data collection process, 
enhance the practical significance of this research area, paving a new way for human avatar reconstruction and real-world applications.



==> Tables/tab_comp_old.tex <==
% \begin{table*}[t]
% \small
% \renewcommand{\arraystretch}{1.1}
% % \setlength\tabcolsep{2pt}
% \centering
% \begin{tabular}{c | c c c | c c c | c c c | c c c }
% \hline
% \multirow{2}{*}{Method}  & \multicolumn{3}{c|}{2-view}  & \multicolumn{3}{c|}{4-view} & \multicolumn{3}{c|}{6-view} & \multicolumn{3}{c}{8-view} \\
%         & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM \\
% \hline 
% & \multicolumn{12}{c}{\textit{FS-XHumans}} \\
% SelfRecon \cite{bib:SelfRecon} \\
% TeCH \cite{bib:TeCH} \\
% ours \\
% \hline
% & \multicolumn{12}{c}{\textit{FS-DART}} \\
% SelfRecon \cite{bib:SelfRecon} \\
% TeCH \cite{bib:TeCH} \\
% ours \\
% \hline
% \end{tabular}
% \caption{Comparison with prior arts on few-shot human reconstruction.}
% \label{tab:comp}
% % \vspace{-0.1cm}
% \end{table*}

\begin{table*}[t]
\small
\renewcommand{\arraystretch}{1.1}
% \setlength\tabcolsep{2pt}
\centering
\begin{tabular}{c | c c c | c c c | c c c }
\hline
\multirow{2}{*}{Method}  & \multicolumn{3}{c|}{2-view}  & \multicolumn{3}{c|}{4-view} & \multicolumn{3}{c}{8-view} \\
        & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS & PSNR & SSIM \\
\hline 
& \multicolumn{9}{c}{\textit{FS-XHumans}} \\
SelfRecon \cite{bib:SelfRecon} \\
TeCH \cite{bib:TeCH} \\
ours \\
\hline
& \multicolumn{9}{c}{\textit{FS-DART}} \\
SelfRecon \cite{bib:SelfRecon} \\
TeCH \cite{bib:TeCH} \\
ours \\
\hline
\end{tabular}
\caption{Comparison with prior arts on few-shot human reconstruction.}
\label{tab:comp}
% \vspace{-0.1cm}
\end{table*}
